Learning to Transform Dynamically for Better Adversarial Transferability

Adversarial examples, crafted by adding perturbations imperceptible to humans, can deceive neural networks. Recent studies identify the adversarial transferability across various models, \textit{i.e.}, the cross-model attack ability of adversarial samples. To enhance such adversarial transferability, existing input transformation-based methods diversify input data with transformation augmentation. However, their effectiveness is limited by the finite number of available transformations. In our study, we introduce a novel approach named Learning to Transform (L2T). L2T increases the diversity of transformed images by selecting the optimal combination of operations from a pool of candidates, consequently improving adversarial transferability. We conceptualize the selection of optimal transformation combinations as a trajectory optimization problem and employ a reinforcement learning strategy to effectively solve the problem. Comprehensive experiments on the ImageNet dataset, as well as practical tests with Google Vision and GPT-4V, reveal that L2T surpasses current methodologies in enhancing adversarial transferability, thereby confirming its effectiveness and practical significance. The code is available at https://github.com/RongyiZhu/L2T.

==> figs/iteration2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/iteration2.pdf}
    \caption{Experiment on copies}
    \label{fig:iteraion2}
\end{figure}

==> figs/lr_p.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/lr&p.pdf}
    \caption{lr\&p}
    \label{fig:method}
\end{figure}

==> figs/motivation.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/motivation.pdf}
    \caption{We show the transferability of adversarial examples in different steps. We use MI-FGSM as the attack algorithm and the ResNet-18 as surrogate model to generate the adversarial examples. We test the Attack Success Rate (ASR) on nine models (ResNet-101, ResNext-50, DenseNet-101, Inception v3, Inception v4, ViT-B\cite{dosovitskiy2020image}, PiT-B, Visformer-S\cite{Chen_2021_ICCV}, Swin-T\cite{liu2021swin}) and show the average ASR on 1000 randomly sample images from ILSVRC 2012 validation set. In the left side column, we set the number of iteration $t$ in MI-FGSM as 1 and apply different transformation operation to the input images. For the four columns on the right, we choose the number of iteration $t$ as 2 and use a fixed transformation operation for the first iteration. We test the influence of different transformation operation on the second iterations. }
    \label{fig:motivation}
\end{figure*}

==> tabs/albation.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule
Method    & ResNet-18 & ResNet101 & ResNeXt-50 & DenseNet-121 & Inception-v3 & Inception-v4 & ViT  & PiT  & Visformer & Swin & Avg  \\ \midrule
L2A       & 100       & 99.2      & 99.2       & 99.5         & 96.7         & 97.3         & 62.9 & 69.7 & 87.0      & 85.8 & 89.7 \\
-Rotate    & 99.7      & 92.4      & 93.9       & 95.7         & 90.3         & 92.4         & 38.2 & 48.2 & 67.9      & 69.1 & 78.8 \\
-Scale     & 99.6      & 90        & 92.3       & 95           & 88.0         & 90.9         & 35.1 & 44.4 & 62.6      & 63.8 & 76.2 \\
-Resize    & 99.9      & 96.4      & 97         & 98.4         & 94.3         & 95.4         & 45.7 & 55.2 & 75.3      & 74.5 & 83.2 \\
-Shuffle   & 99.9      & 95.6      & 95.5       & 97.5         & 93.1         & 94.0         & 39.8 & 51.2 & 71.5      & 71.5 & 81.0 \\
-Mixup     & 100       & 98.7      & 97.6       & 98.8         & 96.6         & 96.7         & 56.8 & 61.4 & 80.5      & 79.6 & 86.7 \\
-Dropout   & 99.7      & 94.8      & 95.2       & 97.6         & 92.5         & 93.3         & 49.5 & 56.7 & 71.3      & 72.5 & 82.3 \\
-Mask      & 99.7      & 91.2      & 91.7       & 95.3         & 89.1         & 90.4         & 35.1 & 45.8 & 63.5      & 66.2 & 76.8 \\
-Spectrum  & 100       & 90.5      & 92.2       & 95.3         & 88.6         & 90.8         & 30.9 & 42.7 & 61.6      & 64.1 & 75.7 \\
-Crop      & 100       & 90.7      & 92.1       & 95.5         & 88.8         & 91.2         & 31.2 & 41   & 60.3      & 64   & 75.5 \\
-Translate & 100       & 99.1      & 98.2       & 99.4         & 96.0         & 95.9         & 51.5 & 61.8 & 82.2      & 80.7 & 86.5 \\ \bottomrule
\end{tabular}}
\end{table}

==> tabs/baseline.tex <==
\begin{table*}[]
%\resizebox{\textwidth}{!}{
\centering
\begin{tabular}{ccccccccccc}
\hline
%Attack & ResNet-18 & ResNet-101 & ResNeXt-50 & DenseNet-121 & Inception-v3 & Inception-v4 & ViT  & PiT  & Visformer & Swin \\ 
Attack & R18 & R101 & RX50 & D121 & Iv3 & Iv4 & ViT  & PiT  & Visformer & Swin \\
\hline
SIM    & 66.5     & 68.2      & 62.9       & 70.4     & 47.6        & 59.5        & 61.5 & 62.3 & 71.3      & 48.5 \\
TIM    & 49.6     & 52.2      & 48.5       & 52.6     & 35.9        & 38.7        & 48.0 & 47.2 & 55.5      & 54.6 \\
$Admix$  & 71.9     & 74.7      & 71.5       & 76.8     & 55.4        & 65.8        & 66.6 & 64.0 & 75.9      & 51.1 \\
DEM    & 79.6     & 81.2      & 81.2       & 82.8     & 64.0        & 67.1        & 82.1 & 80.5 & 84.3      & 78.9 \\
AutoMA & 78.6     & 80.9      & 76.8       & 80.7     & 56.7        & 63.4        & 76.6 & 74.8 & 82.6      & 82.2 \\
IDE    & 53.5     & 56.5      & 54.6       & 64.7     & 42.9        & 46.5        & 66.8 & 68.2 & 76.2      & 62.2 \\
ATTA   & 40.9     & 39.9      & 33.6       & 40.5     & 23.1        & 25.5        & 41   & 40.3 & 47.5      & 37.1 \\
MaskBlock  & 57.0     & 59.4      & 56.3       & 62.1     & 45.6        & 49.2        & 56.7 & 59.4 & 61.8      & 44.2 \\
AITL   & 80.7     & 84.9      & 80.9       & 83.7     & 65.7        & 71.9        & 79.4 & 82.7 & 87.3      & 87.7 \\
$\rm S^2$I    & 73.4     & 78.5      & 79.8       & 83.8     & 61.1        & 66.3        & 71.2 & 73.9 & 82.5      & 81.4 \\
BSR    & 83.0     & 85.9      & 82.8       & 85.7     & 76.7        & 75.3        & 87.3 & 82.9 & 85.9      & 83.0 \\
SIA    & 82.3     & 82.8      & 81.4       & 85.0     & 68.2        & 70.5        & 84.0 & 83.3 & 86.9      & 79.3 \\
\rowcolor[HTML]{C0C0C0} 
L2A    & 90.0       & 91.9      & 91         & 92.8     & 78.8        & 82.4        & 90.1 & 93.5 & 96.2      & 93.6 \\ \hline
\end{tabular}
\end{table*}

==> tabs/method_compare.tex <==

%\begin{table}[]
%\begin{tabular}{llll}
%Method    & Training Time & Training Data                  &  dynamic transformation between iterations  \\
%AutoMA    &               & 1000 Random from ImageNet validation set                          &  \\
%ATTA      &               & 1000 Random Images from ILSVRC 2012 \cite{ILSVRC15} training partition &  \\
%AITL      &               & 1000 ImageNet Images           &  \\
%Ours(L2A) &               &                                & 
%\end{tabular}
%\end{table}


\begin{table}[]
\centering
\begin{tabular}{cccc}
\toprule
Method    & \thead{Additional \\ Training} & \thead{Prior \\ Knowledge}          & \thead{Adaptive to \\ iterations} \\
\midrule
AutoMA    &   \Checkmark      &     \Checkmark         &  \XSolidBrush\\
ATTA      &    \Checkmark      &    \Checkmark            & \XSolidBrush \\
AITL      &    \Checkmark      &    \Checkmark             & \XSolidBrush \\
Ours(L2A) &     \XSolidBold                &    \XSolidBold                       & \CheckmarkBold  \\
\bottomrule
\end{tabular}
\caption{Comparison between different Learn-based algorithm. }
\end{table}
